Leveraging tensor kernels to reduce objective function mismatch in deep clustering

Objective Function Mismatch (OFM) occurs when the optimization of one objective has a negative impact on the optimization of another objective. In this work we study OFM in deep clustering, and find that the popular autoencoder-based approach to deep clustering can lead to both reduced clustering performance, and a significant amount of OFM between the reconstruction and clustering objectives. To reduce the mismatch, while maintaining the structure-preserving property of an auxiliary objective, we propose a set of new auxiliary objectives for deep clustering, referred to as the Unsupervised Companion Objectives (UCOs). The UCOs rely on a kernel function to formulate a clustering objective on intermediate representations in the network. Generally, intermediate representations can include other dimensions, for instance spatial or temporal, in addition to the feature dimension. We therefore argue that the na\"ive approach of vectorizing and applying a vector kernel is suboptimal for such representations, as it ignores the information contained in the other dimensions. To address this drawback, we equip the UCOs with structure-exploiting tensor kernels, designed for tensors of arbitrary rank. The UCOs can thus be adapted to a broad class of network architectures. We also propose a novel, regression-based measure of OFM, allowing us to accurately quantify the amount of OFM observed during training. Our experiments show that the OFM between the UCOs and the main clustering objective is lower, compared to a similar autoencoder-based model. Further, we illustrate that the UCOs improve the clustering performance of the model, in contrast to the autoencoder-based approach. The code for our experiments is available at https://github.com/danieltrosten/tk-uco.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> fig/deep_clustering/ae.tex <==
%!TEX root = main.tex

\begin{tikzpicture}
  \scriptsize
  \tikzNN[
    % Prefix of name
    name={NN},
  	% How the network is built (number of neurons in index layer)
  	nn neurons={3,5,2,2,5,3},
    % Default style of layer rectangles
  	inside layer style={fill=blue!40},
  	% Styles per layer (the rectangle)
  	% layer styles={{fill=red!40},{fill=green!40}},
  	% Scale of whole thing
  	scale={1},
  	% Distance between neuron and layer rectangle
  	layer padding={0.05cm},
  	% How tall the layers are
  	layer height={3cm},
  	% Horisontal separation of layers
  	layer sep={1.5cm},
  	% Size of neurons
  	neuron radius={0.2cm},
  	% Tikz styles
    % Style of the connection between neurons
  	connection style={red},
  	% Color of the neurons
  	neuron color={gray!50},
  	% Node style for neuron
  	neuron style={},
    % Args to send to \begin{scope}
    tikz args={},
    % Show the coordinate names of the layers and neurons
    % verbose=true,
  ];

  \draw[draw=white,fill=white] ($(NN-rectangle-2.south east)+(0.005cm,0)$) rectangle ($(NN-rectangle-3.north west)+(-0.005cm,0)$);

  \def\arrowShorten{3pt}
  \draw [->,shorten >= \arrowShorten,shorten <= \arrowShorten] (NN-rectangle-2.east) -- (NN-rectangle-3.west) node [midway,above] { \( \vec h \)};
  \draw [<-,shorten >= \arrowShorten,shorten <= \arrowShorten] (NN-rectangle-0.west) --++ (-1,0) node [midway,above] {\( \mat X \)};

  \draw [->,shorten >= \arrowShorten,shorten <= \arrowShorten] (NN-rectangle-5.east) --++ (1,0) node [midway,above] {\( \hat{\mat X} \)};

  % \draw [densely dashed, rounded corners, fill=gray, fill opacity=0.25] ($(k1in)+(-1.7,.2)$) rectangle ++(7.0,-3.5);
  \def\boxBuf{3pt}
  \draw [rounded corners, fill=gray, fill opacity=0.25] ($(NN-rectangle-0.north west)+(-\boxBuf,\boxBuf)$)
    rectangle ($(NN-rectangle-2.south east)+(\boxBuf,-\boxBuf)$);
  \node at ($(NN-rectangle-1.south)+(0,-0.3cm)$) {Encoder};

  \draw [rounded corners, fill=gray, fill opacity=0.25] ($(NN-rectangle-3.north west)+(-\boxBuf,\boxBuf)$)
    rectangle ($(NN-rectangle-5.south east)+(\boxBuf,-\boxBuf)$);

  \node at ($(NN-rectangle-4.south)+(0,-0.3cm)$) {Decoder};




\end{tikzpicture}


==> fig/deep_clustering/spectralnet.tex <==
%!TEX root = ../../main.tex

\begin{tikzpicture}
  \pgfdeclarelayer{background}
  \pgfsetlayers{wallpaper,background,main}

  \tikzNN[
    % Prefix of name
    name={NN},
  	% How the network is built (number of neurons in index layer)
  	nn neurons={3,3,3,3},
    % Default style of layer rectangles
  	inside layer style={fill=blue!40},
  	% Styles per layer (the rectangle)
  	% layer styles={{fill=red!40},{fill=green!40}},
  	% Scale of whole thing
  	scale={1},
  	% Distance between neuron and layer rectangle
  	layer padding={0.05cm},
  	% How tall the layers are
  	layer height={3cm},
  	% Horisontal separation of layers
  	layer sep={1.5cm},
  	% Size of neurons
  	neuron radius={0.2cm},
  	% Tikz styles
    % Style of the connection between neurons
  	connection style={red},
  	% Color of the neurons
  	neuron color={gray!50},
  	% Node style for neuron
  	neuron style={},
    % Args to send to \begin{scope}
    tikz args={},
    % Show the coordinate names of the layers and neurons
    % verbose=true,
  ]

  \node at ($(NN-neur-1-0)-(0,1cm)$) {\( f_{\v \theta} \)};
  \node at ($(NN-neur-3-0)-(0,1cm)$) {\( \mat O \)};
  \node at ($(NN-neur-2-0)+(0.85cm,-0.25cm)$) {\( \tilde{\v y} \)};
  \coordinate (L) at ($(NN-neur-3-1)+(0.75cm,0)$);
  \draw[->,very thick] ($(NN-neur-3-1)+(0.25cm,0)$) -- (L) node[midway,above]{\( \v y \)};
  \node[anchor=west] at (L) {\( \cl L \)};
  \draw[<-,very thick] ($(NN-neur-0-1)-(0.5cm,0)$) --++(-0.5,0) node[anchor=east] {\( \v x \)};


  \begin{pgfonlayer}{wallpaper}
    \draw[fill=blue!20] ($(NN-neur-0-2)+(-0.5cm,0.75cm)$) rectangle ($(NN-neur-2-0)+(0.5cm,-0.75cm)$);
  \end{pgfonlayer}

\end{tikzpicture}


==> fig/lambdas/loss.tex <==
% This file was created by matplotlib2tikz v0.6.17.
\begin{tikzpicture}

\begin{axis}[
xlabel={\( \lambda \)},
ylabel={Loss},
xmin=5.01187233627274e-07, xmax=1.99526231496888,
ymin=0.503640118194156, ymax=0.595157517922729,
xmode=log,
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
y grid style={white!69.01960784313725!black},
legend style={at={(0.03,0.97)}, anchor=north west, draw=white!80.0!black},
legend cell align={left},
legend entries={{Best},{Mean \( \pm \) Sd.}}
]
\addlegendimage{no markers, black}
\addlegendimage{no markers, blue}
\path [draw=blue, semithick] (axis cs:1,0.538882363883115)
--(axis cs:1,0.590997636116885);

\path [draw=blue, semithick] (axis cs:0.1,0.509993785646517)
--(axis cs:0.1,0.519856214353483);

\path [draw=blue, semithick] (axis cs:0.01,0.513105616980019)
--(axis cs:0.01,0.527084383019981);

\path [draw=blue, semithick] (axis cs:0.001,0.516295462414422)
--(axis cs:0.001,0.532784537585578);

\path [draw=blue, semithick] (axis cs:0.0001,0.51387054987554)
--(axis cs:0.0001,0.52750945012446);

\path [draw=blue, semithick] (axis cs:1e-05,0.511354938510455)
--(axis cs:1e-05,0.525585061489544);

\path [draw=blue, semithick] (axis cs:1e-06,0.514449722800497)
--(axis cs:1e-06,0.524190277199503);

\addplot [semithick, black, mark=*, mark size=3, mark options={solid}]
table {%
1 0.5286
0.1 0.5078
0.01 0.5089
0.001 0.5113
0.0001 0.5126
1e-05 0.5081
1e-06 0.5113
};
\addplot [semithick, blue, mark=-, mark size=3, mark options={solid}, only marks, forget plot]
table {%
1 0.538882363883115
0.1 0.509993785646517
0.01 0.513105616980019
0.001 0.516295462414422
0.0001 0.51387054987554
1e-05 0.511354938510455
1e-06 0.514449722800497
};
\addplot [semithick, blue, mark=-, mark size=3, mark options={solid}, only marks, forget plot]
table {%
1 0.590997636116885
0.1 0.519856214353483
0.01 0.527084383019981
0.001 0.532784537585578
0.0001 0.52750945012446
1e-05 0.525585061489544
1e-06 0.524190277199503
};
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}, forget plot]
table {%
1 0.56494
0.1 0.514925
0.01 0.520095
0.001 0.52454
0.0001 0.52069
1e-05 0.51847
1e-06 0.51932
};
\end{axis}

\end{tikzpicture}

==> fig/tensor/batchNorm.tex <==
%!TEX root = main.tex

\pgfmathsetmacro{\cubex}{2}
\pgfmathsetmacro{\cubey}{2}
\pgfmathsetmacro{\cubez}{2}
\draw [draw=black, every edge/.append style={draw=black, densely dashed, opacity=.5}, fill=lightgray, fill opacity=0.5]
  (0,0,0) coordinate (o) -- ++(-\cubex,0,0) coordinate (a) -- ++(0,-\cubey,0) coordinate (b) edge coordinate [pos=1] (g) ++(0,0,-\cubez)  -- ++(\cubex,0,0) coordinate (c) -- cycle
  (o) -- ++(0,0,-\cubez) coordinate (d) -- ++(0,-\cubey,0) coordinate (e) edge (g) -- (c) -- cycle
  (o) -- (a) -- ++(0,0,-\cubez) coordinate (f) edge (g) -- (d) -- cycle;
\path [every edge/.append style={draw=black, |-|}]
  (b) +(0,-5pt) coordinate (b1) edge ["\( D_2 \)"'] (b1 -| c)
  (b) +(-5pt,0) coordinate (b2) edge ["\( D_1 \)"] (b2 |- a)
  (c) +(3.5pt,-3.5pt) coordinate (c2) edge ["\( D_3 \)"'] ([xshift=3.5pt,yshift=-3.5pt]e)
  ;
\path (o) -- (b) node [midway] {\( \mat Y \)};


\pgfmathsetmacro{\cubex}{.5}
\pgfmathsetmacro{\cubey}{.5}
\pgfmathsetmacro{\cubez}{2}
\draw [draw=black, every edge/.append style={draw=black, densely dashed, opacity=.5}, fill=lightgray, fill opacity=0.5]
  (-1.5,0,0) coordinate (o) -- ++(-\cubex,0,0) coordinate (a) -- ++(0,-\cubey,0) coordinate (b) edge coordinate [pos=1] (g) ++(0,0,-\cubez)  -- ++(\cubex,0,0) coordinate (c) -- cycle
  (o) -- ++(0,0,-\cubez) coordinate (d) -- ++(0,-\cubey,0) coordinate (e) edge (g) -- (c) -- cycle
  (o) -- (a) -- ++(0,0,-\cubez) coordinate (f) edge (g) -- (d) -- cycle;
\path (a) -- (d) node [midway] {\scriptsize \( \vec y_1 \)};

\pgfmathsetmacro{\cubex}{.5}
\pgfmathsetmacro{\cubey}{.5}
\pgfmathsetmacro{\cubez}{2}
\draw [draw=black, every edge/.append style={draw=black, densely dashed, opacity=.5}, fill=lightgray, fill opacity=0.5]
  (-1,0,0) coordinate (o) -- ++(-\cubex,0,0) coordinate (a) -- ++(0,-\cubey,0) coordinate (b) edge coordinate [pos=1] (g) ++(0,0,-\cubez)  -- ++(\cubex,0,0) coordinate (c) -- cycle
  (o) -- ++(0,0,-\cubez) coordinate (d) -- ++(0,-\cubey,0) coordinate (e) edge (g) -- (c) -- cycle
  (o) -- (a) -- ++(0,0,-\cubez) coordinate (f) edge (g) -- (d) -- cycle;
\path (a) -- (d) node [midway] {\scriptsize \( \vec y_2 \)};

\pgfmathsetmacro{\cubex}{.5}
\pgfmathsetmacro{\cubey}{.5}
\pgfmathsetmacro{\cubez}{2}
\draw [draw=black, every edge/.append style={draw=black, densely dashed, opacity=.5}, fill=lightgray, fill opacity=0.5]
  (0,-1.5,0) coordinate (o) -- ++(-\cubex,0,0) coordinate (a) -- ++(0,-\cubey,0) coordinate (b) edge coordinate [pos=1] (g) ++(0,0,-\cubez)  -- ++(\cubex,0,0) coordinate (c) -- cycle
  (o) -- ++(0,0,-\cubez) coordinate (d) -- ++(0,-\cubey,0) coordinate (e) edge (g) -- (c) -- cycle
  (o) -- (a) -- ++(0,0,-\cubez) coordinate (f) edge (g) -- (d) -- cycle;
\path (a) -- (d) node [midway, xshift=2, yshift=2] {\scriptsize \( \vec y_m \)};


==> inputs/experiments/networkTable.tex <==
%!TEX root = ../../main.tex

\begin{tabular}{cc}\toprule
  \multirow{6}{*}{\minitable{c}{Convolutional\\block 1}} & Convolution (\( 5 \times 5 \times 32 \)) \\
  & \( \relu \) \\
  & Convolution (\( 5 \times 5 \times 32 \)) \\
  & Batch normalization \\
  & \( \relu \) \\
  & MaxPool \\ \midrule
  \multirow{6}{*}{\minitable{c}{Convolutional\\block 2}} & Convolution (\( 3 \times 3 \times 32 \)) \\
  & \( \relu \) \\
  & Convolution (\( 3 \times 3 \times 32 \)) \\
  & Batch normalization \\
  & \( \relu \) \\
  & MaxPool \\ \midrule
  \multirow{4}{*}{\minitable{c}{Fully-connected\\layer 1}} & Flatten \\
  & Fully-connected (\( 100 \)) \\
  & \( \relu \) \\
  & Batch normalization \\ \midrule
  \multirow{2}{*}{\minitable{c}{Output layer/\\Clustering module}} & Fully-connected (\( k \)) \\
  & Softmax \\ \bottomrule
\end{tabular}


==> inputs/experiments/sigmaFig.tex <==
%!TEX root = ../../main.tex

\def\datasetTitleSkip{0.5em}

\begin{subfigure}{\linewidth}
  \begin{minipage}{0.49\linewidth}
    \centering
    {\small \qquad MNIST}
    % \vspace{\datasetTitleSkip}
    \resizeinput{fig/sigmas/MNIST_acc}
  \end{minipage}
  \begin{minipage}{0.49\linewidth}
    \centering
    {\small \qquad USPS}
    % \vspace{\datasetTitleSkip}
    \resizeinput{fig/sigmas/USPS_acc}
  \end{minipage}
  % \begin{minipage}{0.49\linewidth}
  %   \centering
  %   {\small \qquad COIL-20}
  %   % \vspace{\datasetTitleSkip}
  %   \resizeinput{fig/sigmas/COIL-20_acc}
  % \end{minipage}
  \caption{Accuracy}
  \label{fig:sigmas_acc}
\end{subfigure}
\vspace{0.5cm}

\begin{subfigure}{\linewidth}
  \begin{minipage}{0.49\linewidth}
    \centering
    {\small \qquad MNIST}
    \vspace{\datasetTitleSkip}

    \resizeinput{fig/sigmas/MNIST_loss}
  \end{minipage}
  \begin{minipage}{0.49\linewidth}
    \centering
    {\small \qquad USPS}
    \vspace{\datasetTitleSkip}

    \resizeinput{fig/sigmas/USPS_loss}
  \end{minipage}
  % \begin{minipage}{0.49\linewidth}
  %   \centering
  %   {\small \qquad COIL-20}
  %   \vspace{\datasetTitleSkip}
  %
  %   \resizeinput{fig/sigmas/COIL-20_loss}
  % \end{minipage}
  \caption{\( \cl L_\text{DDC} \)}
  \label{fig:sigmas_loss}
\end{subfigure}


==> inputs/method/motivation.tex <==
%!TEX root = ../../main.tex

\commentM{The method section consists of quite a few components right now that can appear a bit disconnected to the reader. You can add some more motivation here in the intro of the section but it might also make sense to split it into more sections and/or change the heading to DTKC. The same I would do in the experiment parts and split the sequential data experiments into an own section (maybe even the hyperparameter analysis).}

\commentY{Find a better place for this, or remove?}
The representational power of deep learning architectures is a double-edged sword when training deep clustering algorithms \cite{guo_improved_2017}. Although these models are indeed capable of producing vectorial representations from noisy and complex data types, they are also capable of drastically changing the between-sample similarities present in the dataset. The majority of deep clustering algorithms rely on the similarities computed from the network's output, meaning that one must adequately regularize the model such that input-similarities are somehow reflected in the output-similarities. Much work focuses on implementing this constraint through the use of autoencoders, where an additional clustering module is attached to the autoencoder's code space \cite{yang_towards_2017,guo_improved_2017,li_discriminatively_2018}. Recall that also the aforementioned DEC \cite{xie_unsupervised_2016} pre-trains the embedding network as an autoencoder (using a reconstruction loss), and then fine-tunes the network using the clustering loss. Thus, the well known DEC also falls within the autoencoder-employing category of algorithms. However, the autoencoder is trained to reconstruct its input as best as possible, meaning that it does not necessarily produce representations suitable for clustering. \commentM{add cite}

Even though the autoencoder approach is a popular one, there are algorithms that do well without the extra guidance provided by the reconstruction loss. Examples of such algorithms include SpectralNet \cite{shaham_spectralnet_2018} and DDC \cite{kampffmeyer_deep_2019}, which were both described earlier in this paper. \commentM{Maybe just say "...reconstruction loss, such as for example SpectralNet ref and DDC ref} These algorithms are trained end-to-end using randomly initialized parameters without explicit regularization terms\footnote{It should be noted however, that DDC's second loss term introduces a regularizing effect to the hidden representation.}. The ability to do without the autoencoder has the benefit of reducing the number of model parameters, potentially increasing training efficiency. Moreover, the end user does not have to worry about pre-training vs. fine-tuning, and other potential difficulties that might arise when combining the autoencoder and the clustering module. However, as is also the case with the autoencoder-based models, these algorithms are far from perfect. In DDC the authors state that the algorithm is indeed prone to getting stuck in local minima, potentially converging to sub-optimal clusterings.


==> inputs/method/self-supervised.tex <==
%!TEX root = ../../main.tex

Self-supervised learning \cite{doersch_unsupervised_2015} is an approach to learning image representations in an unsupervised manner. The main idea is to construct a model that can be trained in a supervised fashion, based on an unlabeled dataset. One approach to this is through the task of \emph{context prediction}, where the model learns to predict the location of an image patch, relative to another patch extracted from the same image. This approach to self-supervised learning is the one we will use throughout this paper. In \cite{doersch_unsupervised_2015}, they argue that a model which is trained to perform this task learns to recognize characteristic parts of the objects present in the dataset. This is indeed intuitive as determining the relative location of one patch with respect to another becomes much easier when one is able to identify the object in the image.

\subsubsection{Model description}
  \begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/selfSupervised/cat}
    \caption[Input to the self-supervised model.]{Input to the self-supervised model. Figure from \cite{doersch_unsupervised_2015}}
    \label{fig:selfSupervised_cat}
  \end{figure}

  The model used for the prediction task is a convolutional neural network, followed by a number of fully-connected layers. The input to the model is illustrated in Figure \ref{fig:selfSupervised_cat}. Note that the different patches outlined in Figure \ref{fig:selfSupervised_cat} are not contiguous, but rather separated and jittered relative to each other. This is done to avoid ``trivial'' solutions where the model simply learns to continue patterns or textures in the image.

  The input \( \mat X \) consists of the two image-patches, which are processed independently by the convolutional layers of the model, as well as the first fully connected layer. Note that the output of the last convolutional layer has to be vectorized (flattened) before being processed by the fully-connected layer. The vectorial representations produced for the two patches by the first fully connected layer are then concatenated, and processed by three more fully-connected layers. The last of these layers produces an \( 8 \)-dimensional vector containing the predicted probabilities of the different relative positions.

  When training the model, these probabilities are compared with the correct position (position \( 3 \) in the example of Figure \ref{fig:selfSupervised_cat}), so that they agree as best as possible. This can be done using an ordinary supervised loss function, such as the cross-entropy loss function \cite{theodoridis_pattern_2009}:
  \[ \cl L_{ce} = - \sums{i=1}{n}\sums{j=1}{8} \lrp{y_{ij} \ln \frac{\hat y_{ij}}{y_{ij}} + (1-y_{ij}) \ln \frac{1 - \hat y_{ij}}{1-y_{ij}} } \]
  where \( n \) is the number of patch-pairs, \( \hat y_{ij} \) is the predicted probability of patch-pair \( i \) having relative position \( j \), and
  \[ y_{ij} = \begin{cases}
      1, &\text{True relative position of pair \( i \) is \( j \)} \\
      0, &\otherwise
    \end{cases}
   \]
   is the one-hot encoded true relative position for patch-pair \( i \).

\subsubsection{From patches to full images}
  The model outlined above is designed to process patches extracted from a given image, rather than the full image. Thus, to obtain one representation for the whole image, one has to slightly modify the model. Recall that the convolution-operator does not require a fixed size input, meaning that the convolutional layers of the model can be left as-is. The fully-connected layers following the concatenation can be discarded, since we only have one image, and thus, nothing to concatenate. This leaves the first fully connected layer, which still requires an input with fixed dimensionality. This layer is transformed to a convolutional layer following \cite{long_fully_2015}. The transformation removes the vectorization-step after the last convolutional layer, and replaces the first fully-connected layer with an equivalent convolutional layer, whose parameters are obtained from the weight matrix belonging to the fully-connected layer it replaces. After this modification, the model is capable of processing an input image of arbitrary size.

  The transformed model can now be used as a feature extractor directly, or to initialize the parameters of another convolutional neural network designed for other image-processing tasks.


==> tab/char_arab.tex <==
\begin{tabularx}{\tableWidth}{c|GGGG|GGGG}
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}Character Trajectories}\\
\hline
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\
\hline
\(k\)-means&\(\mathbf{0.84}\)&\(\mathbf{0.8}\)&\(0.05\)&\(\mathbf{0.86}\)&\(\mathbf{0.86}\)&\(\mathbf{0.86}\)&\(0.03\)&\(\mathbf{0.91}\)\\
Hierarchical&\(0.51\)&\(0.51\)&\(0.0\)&\(0.51\)&\(0.73\)&\(0.73\)&\(0.0\)&\(0.73\)\\
Spectral&\(0.79\)&\(0.78\)&\(0.0\)&\(0.79\)&\(\mathbf{0.86}\)&\(0.85\)&\(0.0\)&\(0.86\)\\
RDDC&\(0.64\)&\(0.58\)&\(0.09\)&\(0.71\)&\(0.73\)&\(0.68\)&\(0.09\)&\(0.81\)\\
R\modelName&\(0.8\)&\(0.65\)&\(0.08\)&\(0.8\)&\(0.83\)&\(0.74\)&\(0.06\)&\(0.83\)\\
\hline
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}Arabic Digits}\\
\hline
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\
\hline
\(k\)-means&\(0.71\)&\(\mathbf{0.67}\)&\(0.05\)&\(0.72\)&\(0.6\)&\(0.6\)&\(0.02\)&\(0.61\)\\
Hierarchical&\(0.1\)&\(0.1\)&\(0.0\)&\(0.1\)&\(0.03\)&\(0.03\)&\(0.0\)&\(0.03\)\\
Spectral&\(0.64\)&\(0.65\)&\(0.02\)&\(0.68\)&\(0.59\)&\(0.58\)&\(0.01\)&\(0.59\)\\
RDDC&\(0.46\)&\(0.55\)&\(0.07\)&\(0.68\)&\(0.63\)&\(\mathbf{0.62}\)&\(0.04\)&\(0.73\)\\
R\modelName&\(\mathbf{0.76}\)&\(0.56\)&\(0.09\)&\(\mathbf{0.76}\)&\(\mathbf{0.74}\)&\(0.61\)&\(0.07\)&\(\mathbf{0.76}\)\\
\hline
\end{tabularx}


==> tab/fmnist_coil20_coil100_umist.tex <==
\begin{tabularx}{\tableWidth}{c|GGGG|GGGG}
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}Fashion-MNIST}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
\(k\)-means&\(0.47\)&\(0.52\)&\(0.04\)&\(0.61\)&\(0.51\)&\(0.51\)&\(0.01\)&\(0.54\)\\
Hierarchical&\(0.1\)&\(0.1\)&\(0.0\)&\(0.1\)&\(0.01\)&\(0.01\)&\(0.0\)&\(0.01\)\\
Spectral&\(0.48\)&\(0.5\)&\(0.02\)&\(0.52\)&\(0.5\)&\(0.5\)&\(0.01\)&\(0.52\)\\
DEC&\(0.56\)&\(0.55\)&\(0.01\)&\(0.58\)&\(0.6\)&\(\mathbf{0.6}\)&\(0.01\)&\(0.62\)\\
DDC&\(0.58\)&\(0.55\)&\(0.06\)&\(0.65\)&\(0.52\)&\(0.49\)&\(0.04\)&\(0.56\)\\
DDC-SS&\(0.57\)&\(\mathbf{0.58}\)&\(0.05\)&\(\mathbf{0.7}\)&\(0.58\)&\(0.58\)&\(0.04\)&\(\mathbf{0.65}\)\\
\modelName&\(0.63\)&\(0.56\)&\(0.04\)&\(0.63\)&\(0.55\)&\(0.5\)&\(0.03\)&\(0.56\)\\
\modelName-SS&\(\mathbf{0.65}\)&\(0.55\)&\(0.05\)&\(0.65\)&\(\mathbf{0.62}\)&\(0.55\)&\(0.03\)&\(0.62\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}COIL-20}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DBC&\(\mathbf{0.79}\)&--&--&--&\(\mathbf{0.9}\)&--&--&--\\
\(k\)-means&\(0.69\)&\(0.63\)&\(0.04\)&\(0.7\)&\(0.8\)&\(0.77\)&\(0.01\)&\(0.8\)\\
Hierarchical&\(0.35\)&\(0.35\)&\(0.0\)&\(0.35\)&\(0.67\)&\(0.67\)&\(0.0\)&\(0.67\)\\
Spectral&\(0.61\)&\(0.65\)&\(0.03\)&\(0.68\)&\(0.76\)&\(0.77\)&\(0.01\)&\(0.78\)\\
DEC&\(0.67\)&\(0.66\)&\(0.04\)&\(0.71\)&\(0.77\)&\(0.77\)&\(0.01\)&\(0.8\)\\
DDC&\(0.68\)&\(0.64\)&\(0.03\)&\(0.71\)&\(0.77\)&\(0.75\)&\(0.03\)&\(0.81\)\\
DDC-SS&\(0.71\)&\(0.67\)&\(0.03\)&\(0.72\)&\(0.81\)&\(\mathbf{0.79}\)&\(0.02\)&\(0.82\)\\
\modelName&\(0.62\)&\(0.64\)&\(0.03\)&\(0.69\)&\(0.75\)&\(0.75\)&\(0.03\)&\(0.8\)\\
\modelName-SS&\(0.71\)&\(\mathbf{0.68}\)&\(0.03\)&\(\mathbf{0.74}\)&\(0.82\)&\(\mathbf{0.79}\)&\(0.02\)&\(\mathbf{0.83}\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}COIL-100}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DBC&\(\mathbf{0.78}\)&--&--&--&\(\mathbf{0.91}\)&--&--&--\\
\(k\)-means&\(0.62\)&\(\mathbf{0.61}\)&\(0.01\)&\(0.63\)&\(0.83\)&\(0.83\)&\(0.0\)&\(0.84\)\\
Hierarchical&\(0.23\)&\(0.23\)&\(0.0\)&\(0.23\)&\(0.68\)&\(0.68\)&\(0.0\)&\(0.68\)\\
Spectral&\(0.44\)&\(0.56\)&\(0.05\)&\(0.61\)&\(0.76\)&\(0.81\)&\(0.02\)&\(0.83\)\\
DEC&\(0.59\)&\(\mathbf{0.61}\)&\(0.02\)&\(\mathbf{0.65}\)&\(0.84\)&\(\mathbf{0.85}\)&\(0.01\)&\(\mathbf{0.86}\)\\
DDC&\(0.61\)&\(0.59\)&\(0.02\)&\(0.63\)&\(0.83\)&\(0.83\)&\(0.01\)&\(0.84\)\\
DDC-SS&\(0.5\)&\(0.49\)&\(0.03\)&\(0.53\)&\(0.78\)&\(0.77\)&\(0.01\)&\(0.79\)\\
\modelName&\(0.64\)&\(0.6\)&\(0.02\)&\(\mathbf{0.65}\)&\(0.85\)&\(0.83\)&\(0.01\)&\(0.85\)\\
\modelName-SS&\(0.51\)&\(0.5\)&\(0.02\)&\(0.52\)&\(0.77\)&\(0.77\)&\(0.01\)&\(0.78\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}UMist}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
\(k\)-means&\(0.4\)&\(0.42\)&\(0.02\)&\(\mathbf{0.46}\)&\(0.59\)&\(0.61\)&\(0.01\)&\(0.64\)\\
Hierarchical&\(\mathbf{0.46}\)&\(\mathbf{0.46}\)&\(0.0\)&\(\mathbf{0.46}\)&\(0.66\)&\(0.66\)&\(0.0\)&\(0.66\)\\
Spectral&\(0.36\)&\(0.42\)&\(0.03\)&\(\mathbf{0.46}\)&\(0.58\)&\(0.63\)&\(0.02\)&\(0.66\)\\
DEC&\(0.08\)&\(0.24\)&\(0.12\)&\(0.4\)&\(\mathbf{1.69}\)&\(\mathbf{0.75}\)&\(0.56\)&\(\mathbf{1.69}\)\\
DDC&\(0.31\)&\(0.36\)&\(0.03\)&\(0.42\)&\(0.46\)&\(0.52\)&\(0.02\)&\(0.55\)\\
DDC-SS&\(0.35\)&\(0.35\)&\(0.02\)&\(0.4\)&\(0.51\)&\(0.51\)&\(0.02\)&\(0.54\)\\
\modelName&\(0.29\)&\(0.36\)&\(0.04\)&\(0.42\)&\(0.45\)&\(0.52\)&\(0.04\)&\(0.59\)\\
\modelName-SS&\(0.34\)&\(0.34\)&\(0.03\)&\(0.41\)&\(0.51\)&\(0.51\)&\(0.03\)&\(0.57\)\\
\hline 
\end{tabularx}

==> tab/mnist_usps_svhn.tex <==
\begin{tabularx}{\tableWidth}{c|GGGG|GGGG}
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}MNIST}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DBC&\(0.96\)&--&--&--&\(\mathbf{0.92}\)&--&--&--\\
DCN&\(0.83\)&--&--&--&\(0.81\)&--&--&--\\
IDEC&\(0.88\)&--&--&--&\(0.87\)&--&--&--\\
SpectralNet&\(\mathbf{0.97}\)&--&--&--&\(\mathbf{0.92}\)&--&--&--\\
\(k\)-means&\(0.51\)&\(0.54\)&\(0.03\)&\(0.58\)&\(0.49\)&\(0.5\)&\(0.01\)&\(0.52\)\\
Hierarchical&\(0.21\)&\(0.21\)&\(0.0\)&\(0.21\)&\(0.31\)&\(0.31\)&\(0.0\)&\(0.31\)\\
Spectral&\(0.5\)&\(0.55\)&\(0.02\)&\(0.56\)&\(0.51\)&\(0.51\)&\(0.01\)&\(0.52\)\\
DEC&\(0.83\)&\(\mathbf{0.87}\)&\(0.03\)&\(\mathbf{0.95}\)&\(0.85\)&\(\mathbf{0.86}\)&\(0.01\)&\(\mathbf{0.89}\)\\
DDC&\(0.91\)&\(0.77\)&\(0.07\)&\(0.91\)&\(0.83\)&\(0.73\)&\(0.06\)&\(0.83\)\\
DDC-SS&\(0.88\)&\(0.76\)&\(0.09\)&\(0.9\)&\(0.83\)&\(0.74\)&\(0.07\)&\(0.84\)\\
\modelName&\(0.94\)&\(0.77\)&\(0.08\)&\(0.94\)&\(0.88\)&\(0.74\)&\(0.07\)&\(0.88\)\\
\modelName-SS&\(0.87\)&\(0.76\)&\(0.07\)&\(0.87\)&\(0.84\)&\(0.74\)&\(0.06\)&\(0.84\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}USPS}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DBC&\(0.74\)&--&--&--&\(0.72\)&--&--&--\\
IDEC&\(0.76\)&--&--&--&\(0.78\)&--&--&--\\
\(k\)-means&\(0.67\)&\(0.63\)&\(0.04\)&\(0.69\)&\(0.63\)&\(0.62\)&\(0.02\)&\(0.65\)\\
Hierarchical&\(0.22\)&\(0.22\)&\(0.0\)&\(0.22\)&\(0.19\)&\(0.19\)&\(0.0\)&\(0.19\)\\
Spectral&\(0.59\)&\(0.65\)&\(0.02\)&\(0.66\)&\(0.6\)&\(0.6\)&\(0.0\)&\(0.61\)\\
DEC&\(0.76\)&\(\mathbf{0.76}\)&\(0.0\)&\(0.77\)&\(0.78\)&\(\mathbf{0.78}\)&\(0.0\)&\(0.79\)\\
DDC&\(\mathbf{0.81}\)&\(0.69\)&\(0.06\)&\(\mathbf{0.83}\)&\(0.77\)&\(0.7\)&\(0.03\)&\(0.77\)\\
DDC-SS&\(0.72\)&\(0.69\)&\(0.05\)&\(0.78\)&\(0.7\)&\(0.7\)&\(0.03\)&\(0.78\)\\
\modelName&\(0.78\)&\(0.7\)&\(0.06\)&\(0.79\)&\(\mathbf{0.8}\)&\(0.73\)&\(0.05\)&\(\mathbf{0.81}\)\\
\modelName-SS&\(0.69\)&\(0.68\)&\(0.05\)&\(0.76\)&\(0.69\)&\(0.69\)&\(0.04\)&\(0.75\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}SVHN}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
\(k\)-means&\(0.13\)&\(0.13\)&\(0.0\)&\(0.13\)&\(0.02\)&\(0.02\)&\(0.0\)&\(0.02\)\\
Hierarchical&\(\mathbf{0.19}\)&\(0.19\)&\(0.0\)&\(0.19\)&\(0.0\)&\(0.0\)&\(0.0\)&\(0.0\)\\
Spectral&\(0.13\)&\(0.14\)&\(0.0\)&\(0.14\)&\(0.02\)&\(0.02\)&\(0.0\)&\(0.02\)\\
DEC&\(0.18\)&\(\mathbf{0.2}\)&\(0.01\)&\(\mathbf{0.23}\)&\(\mathbf{0.07}\)&\(\mathbf{0.09}\)&\(0.02\)&\(\mathbf{0.14}\)\\
DDC&\(0.15\)&\(0.14\)&\(0.01\)&\(0.17\)&\(0.02\)&\(0.02\)&\(0.01\)&\(0.04\)\\
DDC-SS&\(\mathbf{0.19}\)&\(0.18\)&\(0.01\)&\(0.2\)&\(0.06\)&\(0.05\)&\(0.01\)&\(0.08\)\\
\modelName&\(0.17\)&\(0.18\)&\(0.01\)&\(0.21\)&\(0.05\)&\(0.06\)&\(0.01\)&\(0.09\)\\
\modelName-SS&\(0.14\)&\(0.14\)&\(0.01\)&\(0.17\)&\(0.02\)&\(0.02\)&\(0.01\)&\(0.05\)\\
\hline 
\end{tabularx}

==> tab/sm_mnist_fmnist_coil100.tex <==
\begin{tabularx}{\tableWidth}{c|GGGG|GGGG}
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}MNIST}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DDC&\(0.91\)&\(\mathbf{0.77}\)&\(0.07\)&\(0.91\)&\(0.83\)&\(0.73\)&\(0.06\)&\(0.83\)\\
\modelName&\(\mathbf{0.94}\)&\(\mathbf{0.77}\)&\(0.08\)&\(\mathbf{0.94}\)&\(\mathbf{0.88}\)&\(\mathbf{0.74}\)&\(0.07\)&\(\mathbf{0.88}\)\\
\modelName-SM&\(0.87\)&\(\mathbf{0.77}\)&\(0.08\)&\(0.87\)&\(0.84\)&\(\mathbf{0.74}\)&\(0.07\)&\(0.84\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}Fashion-MNIST}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DDC&\(0.58\)&\(0.55\)&\(0.06\)&\(\mathbf{0.65}\)&\(0.52\)&\(0.49\)&\(0.04\)&\(\mathbf{0.56}\)\\
\modelName&\(\mathbf{0.63}\)&\(\mathbf{0.56}\)&\(0.04\)&\(0.63\)&\(\mathbf{0.55}\)&\(\mathbf{0.5}\)&\(0.03\)&\(\mathbf{0.56}\)\\
\modelName-SM&\(0.56\)&\(0.54\)&\(0.05\)&\(0.62\)&\(0.51\)&\(0.49\)&\(0.03\)&\(0.54\)\\
\hline 
\multicolumn{9}{c}{\rule{0pt}{\datasetNameSpace}COIL-100}\\ 
\hline 
&\multicolumn{4}{c|}{ACC} & \multicolumn{4}{c}{NMI} \\ 
Model & Best & Mean & Sd. & Max & Best & Mean & Sd. & Max \\ 
\hline 
DDC&\(0.61\)&\(0.59\)&\(0.02\)&\(0.63\)&\(0.83\)&\(\mathbf{0.83}\)&\(0.01\)&\(0.84\)\\
\modelName&\(\mathbf{0.64}\)&\(\mathbf{0.6}\)&\(0.02\)&\(\mathbf{0.65}\)&\(\mathbf{0.85}\)&\(\mathbf{0.83}\)&\(0.01\)&\(\mathbf{0.85}\)\\
\modelName-SM&\(0.59\)&\(\mathbf{0.6}\)&\(0.02\)&\(0.62\)&\(0.83\)&\(\mathbf{0.83}\)&\(0.01\)&\(\mathbf{0.85}\)\\
\hline 
\end{tabularx}
